High Velocity Kernel File Systems with Bento

High development velocity is critical for modern systems. This is especially true for Linux file systems which are seeing increased pressure from new storage devices and new demands on storage systems. However, high velocity Linux kernel development is challenging due to the ease of introducing bugs, the difficulty of testing and debugging, and the lack of support for redeployment without service disruption. Existing approaches to high-velocity development of file systems for Linux have major downsides, such as the high performance penalty for FUSE file systems, slowing the deployment cycle for new file system functionality. We propose Bento, a framework for high velocity development of Linux kernel file systems. It enables file systems written in safe Rust to be installed in the Linux kernel, with errors largely sandboxed to the file system. Bento file systems can be replaced with no disruption to running applications, allowing daily or weekly upgrades in a cloud server setting. Bento also supports userspace debugging. We implement a simple file system using Bento and show that it performs similarly to VFS-native ext4 on a variety of benchmarks and outperforms a FUSE version by 7x on 'git clone'. We also show that we can dynamically add file provenance tracking to a running kernel file system with only 15ms of service interruption.

==> discussion.tex <==
\section{Future Work}

The work we have done on \system{} so far is the beginning of a larger project. Over the next year, we plan to further work both on \system{} for file systems and for other interfaces across the Linux kernel. Over the next six months, we plan to conclude our work on the file system extensibility layer and submit a paper on the topic. After that, we intend to apply the concepts in this paper to other interfaces across the Linux kernel, starting with networking.

\subsection{Fully Supporting File Systems}
%Our next step is to complete the final work on this project and publish a full paper on it in the next six months. The first step is to implement online reconfiguration in our framework, enabling file systems to be redeployed without shutting down services that rely on the file system. Part of this work will involve cleaning up the framework, making it ready to release to the wider file system development community. We'll also address the additional challenges described in \autoref{sec:goals-challenges} that haven't been previously addressed (composable file systems and a support for a debugging API) and implement real-world file systems as described in \autoref{subsec:real-world}.

%\subsubsection{Linux \texttt{io\_uring}}
On top of addressing the remaining challenges and implementing future work discussed thus far (online upgrades, debugging API, composable file systems, real-world evaluation), we will update to more recent kernel versions to take advantage of new functionality. Recent versions of the Linux kernel have included a new abstraction for performing asynchronous I/O from userspace called \texttt{io\_uring}. Using this interface for the I/O accesses from the FUSE version of the xv6 file system in the evaluation could result in better performance numbers, potentially decreasing the overhead seen by using FUSE. More interestingly, our framework could hook into the file I/O part of \texttt{io\_uring} along with the VFS layer, allowing users to entirely bypass the VFS layer. We cannot currently use \texttt{io\_uring} because our framework is built in Linux kernel version 4.15 and \texttt{io\_uring} requires version 5.1. Updating to the new kernel version and incorporating \texttt{io\_uring} is part of our future work on this project.

\subsection{Beyond File Systems}
While this project focuses on file systems, none of the goals, challenges, or techniques are unique to file systems; other types of extensions can also benefit from this design. We plan to first focus on networking, particularly the TCP/IP functionality (or more broadly, OSI layers 3 and 4). Recent work has shown demand for specialized, userspace network stacks~\cite{snap, 10.1145/2740070.2626311} to improve performance for specific applications. Similarly, exokernel operating systems~\cite{exokernel} and kernel-bypass networking~\cite{arrakis} seek to improve performance by using optimized network stacks and/or avoiding the overhead of the Linux kernel network stack. However, kernel bypass networking has downsides, requiring the whole NIC to be given to the userspace process and burning CPU cores for polling. Applying the concepts from this projects to kernel networking could enable running specialized network stacks in the kernel, enabling the performance gains of running a specialized network stack without the downsides of kernel bypass networking.

In the long term, we intend to apply the concepts from this project to interfaces across the Linux kernel. Many interfaces could benefit from improved safety and increased development velocity. Past work has used Rust to write drivers~\cite{rust_devices}, but these drivers still have a significant amount of unsafe code. Other pieces of the kernel, such as scheduling algorithms or security modules, could be targets for future work.

==> evaluation_old.tex <==
\section{Evaluation}
We evaluate the performance of \system{} to determine what, if any, overheads exist to using it. For this, we have implemented the file system from the xv6 teaching operating system
and two variants:
%to understand how \system{} would affect the performance of this simple file system. We've also implemented two baselines of this file system:
one written in C, running in the kernel using the VFS layer and one written in Rust, running in userspace using FUSE. By comparing against the VFS layer, we can determine the overhead \system{} introduces.
By comparing against FUSE, we can quantify the benefits of \system{} relative to a purely userlevel file system.

%For the macrobenchmarks we run, we additionally compare the three versions of the xv6 file system against ext4. Since xv6 is a toy operating system, it's missing many performance optimizations and isn't able to achieve the performance provided by real-world file systems like ext4. Therefore the performance numbers won't be identical, but can still be compared to understand ballpark performance differences. We mount ext4 with the \texttt{data=journal} option so it logs file data in the journal like the xv6 file system.

Since xv6 is a toy operating system, it is missing optimizations that a commercial-grade optimizations would have. This can heavily impact the FUSE baseline because the unoptimized operations may be particularly expensive from userspace. The VFS baseline is also less optimized than \system{} because \system{} inherits optimizations from the FUSE kernel module while the VFS baseline was just written for this evaluation. Therefore, the xv6 evaluation could be somewhat unfairly optimistic to \system{} when compared to the same evaluation on a commercial-grade file system. We therefore also compare against ext4 on the macrobenchmarks. Ext4 is more optimized than the xv6 file system, but the performance results can still be compared to understand ballpark performance differences. Relatively small differences can indicate that our results may be similar to those we would achieve on a commercial-grade file system. We mount ext4 with the \texttt{data=journal} option so it logs file data in the journal like the xv6 file system.


\subsection{Xv6 File System Changes}
In order to write the xv6 file system in Rust and run the benchmarks, some changes needed to be made to the file system design. In all versions of the file system, we needed to add locks around inode and block number allocations due to race conditions on the block device. We also added double indirect blocks to all three versions of the file system so files up to 4GB could be created. In general, the Rust versions include more locks than the C version and official xv6 repository~\cite{xv6-public}, specifically on global mutable variables that are only modified during initialization. Otherwise, the Rust file systems are nearly identical to the C file systems.

\subsection{Baseline Implementations}
%\todo{this should be part of the eval.}
%To evaluate the performance characteristics of \system{}, we've implemented three versions of the xv6 file system. One version was implemented using \system{} along with two baselines, one running in the kernel using the VFS layer and one running in userspace using FUSE. \system{}'s version of the file system is implemented in 1668 lines of Rust code.

As a baseline, we implement a VFS file system written in C. It is implemented in 1862 lines of C code. This filesystem is as close to our framework’s version as possible to enable accurate comparison between the two approaches. This baseline allows us to analyze any overhead that \system{} may introduce over the VFS layer.

The other baseline is a userlevel version using FUSE.
This is 1744 lines of Rust and uses a Rust reimplementation of the FUSE userspace library~\cite{fuse-rs} with minor changes such as enabling the writeback cache. The code for this version is nearly identical to the code written using our framework. Minor changes to the code are needed to swap out kernel services for Rust user-level services, such as using the Rust standard library mutex instead of the kernel semaphore. Additionally, block I/O from userspace is done by opening the Linux disk file using the \texttt{O\_DIRECT} flag. We note future work will be able to run the same code in \system{} and at userlevel.


\subsection{Test Setup}
The benchmarks were run on a machine with 8 $\times$ Intel Core i7 CPU, 31 GiB DDR4 RAM, and a 512GB Samsung PM981 NVMe SSD. All benchmarks were run using the SSD as the backing device. Due to the present health concerns, the benchmarks were run through a virtual machine using PCIe passthrough to access the SSD.

\subsection{Benchmarks}
%Past work~\cite{tofuse} has evaluated the performance overhead of a FUSE file system using benchmarks from the Filebench benchmark suite. In that work, the FUSE file system forwards requests to a kernel file system, so the evaluation only measures overhead from the FUSE design and doesn't include potential overheads from implementing the file system in userspace. Despite this difference from our evaluation, this work helps by identifying areas where a FUSE file system would show performance degradation over a VFS file system. We use the same benchmarks as that paper to understand the performance characteristics of our framework compared to both FUSE and the VFS layer. We additionally add one extra macrobenchmark (untaring the Linux kernel). These benchmarks cover a wide variety of micro-benchmarks and macro-benchmarks, including both data-intensive and metadata-intensive benchmarks.

From filebench, we run the single-threaded and 32-threaded read, write, file creation and file deletion microbenchmarks and the varmail and fileserver macrobenchmarks. To this, we also measure untaring the Linux kernel. These benchmarks were run on an NVME SSD and executed for one minute in all cases. The varmail macrobenchmark simulates a mail server. It repeatedly generates file creates, file deletes, file reads and writes, and appends to an operation log, syncing after writing.
The fileserver macrobenchmark simulates a file serving application.

%\subsection{FUSE Overhead} \label{subsec:fuse-oh}
We see significant slowdown because of slow block I/O from userspace, even through the \texttt{O\_DIRECT} file interface. Each block operation from userspace must pass across the user/kernel boundary and through the VFS layer before reaching the disk, adding 200-400ns to each operation. On top of that, the file interface imposes additional overheads. The file system must occasionally sync blocks to disk (such as during log operations), but the file interface provides no way to sync parts of a file, so the whole disk file must be synced every time one block needs to be synced, making fsyncs very costly. 

\subsection{Microbenchmarks}
\subsubsection{Read}

\begin{figure}
    \centering
    \input{figures/evaluation/read_4k}
    \caption{Read Performance (4KB), Ops/sec}
    \label{fig:read_4k}
\end{figure}

\begin{figure*}
\begin{subfigure}{\textwidth}
    \centering
    \input{figures/evaluation/legend}
    \label{fig:legend}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
    \centering
    \input{figures/evaluation/read_32k}
    \caption{Reads (32KB)}
    \label{fig:read_32k}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
    \centering
    \input{figures/evaluation/read_128k}
    \caption{Reads (128KB)}
    \label{fig:read_128k}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
    \centering
    \input{figures/evaluation/read_1024k}
    \caption{Reads (1024KB)}
    \label{fig:read_1024k}
\end{subfigure}
\caption{Read Performance (32KB-1024KB), Throughput MBps (x1000)}
\label{read_tp}
\end{figure*}

%\begin{figure*}
%\begin{subfigure}{\textwidth}
%    \centering
%    \input{figures/evaluation/legend}
%    \label{fig:legend}
%\end{subfigure}
%\begin{subfigure}{.24\textwidth}
%    \centering
%    \input{figures/evaluation/seq_read_1t}
%    \caption{Sequential Read, 1 Thread}
%    \label{fig:seq_read_1t}
%\end{subfigure}
%\begin{subfigure}{.24\textwidth}
%    \centering
%    \input{figures/evaluation/seq_read_32t}
%    \caption{Sequential Read, 32 Threads}
%    \label{fig:seq_read_32t}
%\end{subfigure}
%\begin{subfigure}{.24\textwidth}
%    \centering
%    \input{figures/evaluation/rnd_read_1t}
%    \caption{Random Read, 1 Thread}
%    \label{fig:rnd_read_1t}
%\end{subfigure}
%\begin{subfigure}{.24\textwidth}
%    \centering
%    \input{figures/evaluation/rnd_read_32t}
%    \caption{Random Read, 32 Threads}
%    \label{fig:rnd_read_32t}
%\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%    \centering
%    \input{figures/evaluation/seq_read_1t_tp}
%    \caption{Sequential Read, 1 Thread}
%    \label{fig:seq_read_1t_tp}
%\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%    \centering
%    \input{figures/evaluation/seq_read_32t_tp}
%    \caption{Sequential Read, 32 Threads}
%    \label{fig:seq_read_32t_tp}
%\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%    \centering
%    \input{figures/evaluation/rnd_read_1t_tp}
%    \caption{Random Read, 1 Thread}
%    \label{fig:rnd_read_1t_tp}
%\end{subfigure}
%\begin{subfigure}{0.24\textwidth}
%    \centering
%    \input{figures/evaluation/rnd_read_32t_tp}
%    \caption{Random Read, 32 Thread}
%    \label{fig:rnd_read_32t_tp}
%\end{subfigure}
%\caption{Read Performance, Ops/sec and Throughput}
%\label{fig:read}
%\end{figure*}

The performance results for the read microbenchmarks are shown in \autoref{fig:read_4k} and \autoref{read_tp}. All figures include single-threaded and 32-threaded benchmarks for both sequential read and random read. \autoref{fig:read_4k} shows performance for 4KB reads in operations per second. The other graphs show performance for 32KB, 128KB, and 1024 KB reads in throughput, measured in MBps.

All three versions of the file system show very similar performance results for all sizes of reads for both random and sequential reads. The similarity in performance is due to in-kernel caching and the small size of the file. All three versions of the file system use the same technique for caching read requests, implemented in the file system in the C-kernel version, in the file operations layer in \system{}, and in FUSE kernel module for the FUSE version. Since the file is small and read requests are fast, the file is cached very quickly. After this, all requests hit the same in-kernel cache, and all versions execute the exact same code. The xv6 file system cannot support files larger than 4GB, so we cannot run a benchmark that evaluates the differences.


\subsubsection{Write}

%\begin{figure*}
%\begin{subfigure}{\textwidth}
%    \centering
%    \input{figures/evaluation/legend}
%    \label{fig:legend}
%\end{subfigure}
%\begin{subfigure}{.32\textwidth}
%    \centering
%    \input{figures/evaluation/seq_write_1t}
%    \caption{Sequential Write, 1 Thread}
%    \label{fig:seq_write_1t}
%\end{subfigure}
%\begin{subfigure}{.32\textwidth}
%    \centering
%    \input{figures/evaluation/rnd_write_1t}
%    \caption{Random Write, 1 Thread}
%    \label{fig:rnd_write_1t}
%\end{subfigure}
%\begin{subfigure}{.32\textwidth}
%    \centering
%    \input{figures/evaluation/rnd_write_32t}
%    \caption{Random Write, 32 Threads}
%    \label{fig:rnd_write_32t}
%\end{subfigure}
%\begin{subfigure}{.32\textwidth}
%    \centering
%    \input{figures/evaluation/seq_write_1t_tp}
%    \caption{Sequential Write, 1 Thread}
%    \label{fig:seq_write_1t_tp}
%\end{subfigure}
%\begin{subfigure}{.32\textwidth}
%    \centering
%    \input{figures/evaluation/rnd_write_1t_tp}
%    \caption{Random Write, 1 Thread}
%    \label{fig:rnd_write_1t_tp}
%\end{subfigure}
%\begin{subfigure}{.32\textwidth}
%    \centering
%    \input{figures/evaluation/rnd_write_32t_tp}
%    \caption{Random Write, 32 Thread}
%    \label{fig:rnd_write_32t_tp}
%\end{subfigure}
%\caption{Write Performance, Ops/sec and Throughput}
%\label{fig:write}
%\end{figure*}

\begin{figure*}
\begin{subfigure}{\textwidth}
    \centering
    \input{figures/evaluation/legend}
    \label{fig:legend}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
    \centering
    \input{figures/evaluation/write_32k}
    \caption{Writes (32KB)}
    \label{fig:write_32k}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
    \centering
    \input{figures/evaluation/write_128k}
    \caption{Writes (128KB)}
    \label{fig:write_128k}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
    \centering
    \input{figures/evaluation/write_1024k}
    \caption{Writes (1024KB)}
    \label{fig:write_1024k}
\end{subfigure}
\caption{Write Performance, Throughput (MBps)}
\label{fig:write}
\end{figure*}

The performance results for the write microbenchmarks are shown in \autoref{fig:write}. The graphs include single-threaded sequential writes and single-threaded and 32-threaded random writes for 32KB, 128KB and 1024KB writes. Our evaluation does not include 4KB writes because these often triggered a segmentation fault in Filebench. Performance is measured in throughput in MBps. The performance of the FUSE file system was so low, these bars are nearly flush with the bottom of the graphs.

The \system{} file system shows similar performance to the C version of the file system, and both perform much better than the FUSE version of the file system. The versions written in Rust using \system{} and in C in the kernel implement nearly identical behavior, so it is expected for them to have similar performance. The \system{} file system performs somewhat better than the VFS file system on large writes because \system{}, which inherits from the FUSE kernel module, uses a more optimized technique for writing pages. \system{} uses the \texttt{writepages} method instead of \texttt{writepage}, allowing sequential pages to be batched.

We see significant slowdown because of slow block I/O from userspace, even through the \texttt{O\_DIRECT} file interface. Each block operation from userspace must pass across the user/kernel boundary and through the VFS layer before reaching the disk, adding 200-400ns to each operation. On top of that, the file interface imposes additional overheads. The file system must occasionally sync blocks to disk (such as during log operations), but the file interface provides no way to sync parts of a file, so the whole disk file must be synced every time one block needs to be synced, making \texttt{fsync}s very costly.

%Our evaluation shows FUSE having much higher performance overhead than seen in \cite{tofuse} because our FUSE implementation executes block I/O from userspace, introducing significant slowdown. Individual block operations from userspace must pass across the user/kernel boundary and through the VFS layer to reach the block device, adding hundreds of nanoseconds of overhead per operation. The file API used for userspace block I/O also adds overhead. Since whole blocks must be written to an \texttt{O\_DIRECT} file, for partial-block writes, the file system must read the block before writing it, resulting in two operations per write. Additionally, there's no way to sync only part of a file, so any time a block needs to be synced, such as writing to the log, every block must be synced.

%Userspace block I/O, by opening the backing device file with \texttt{O\_DIRECT}, is much slower than kernel block I/O for two main reasons: per-operation overhead and mismatch between the file API and block operations. Each block operation from userspace is much slower than the equivalent block operation from the kernel because the userspace operations must pass across the user/kernel boundary and through the VFS layer, adding 200-400ns of latency to each read or write operation. The file API used to access the backing disk from userspace compounds this issue. Block operations, and file operations on an \texttt{O\_DIRECT} file, are executed at block granularity, requiring the user to write whole blocks at a time. However, the file system may not want to completely overwrite a block. Therefore, the file system must first read the whole block from the file, modify part of the data, and write the whole block back to the disk, turning every write operation into two disk operations, a read and a write. Additionally, blocks must be synced during logging, but the file API provides no way to sync one part of the disk without syncing the whole disk, so the log must sync the whole disk every time.

%Our framework outperforms both of the other versions for sequential writes. For sequential writes, particularly small writes, the C version in the kernel lags behind the framework because it currently uses a different interface for flushing cached writes. The FUSE kernel module, which our framework is based on, batches sequential writes up to 32 pages (sized 4KB). The in-kernel version currently writes each page individually, so doesn't gain the benefit of batching.

%For random writes, our framework shows similar performance to the C version in the kernel, but both have worse performance than the FUSE version, particularly on large writes. The FUSE version shows very high write performance on the RAM disk because \texttt{fsync}s to the RAM disk from userspace are no-ops. The FUSE version uses the file system API to access the disk while the in-kernel file systems instead use the buffer cache for disk accesses. The file system that wraps RAM disks (\texttt{ramfs}) executes a no-op in place of \texttt{fsync}; after all, RAM can't provide persistence. When these benchmarks are run on the SSD, this performance difference should disappear.

%Like reads, we can anticipate that the FUSE version should show significant performance overhead due to slow disk I/O. This is already seen to some extent in sequential writes. Again like reads, this overhead isn't reflected in \cite{tofuse} since that file system didn't execute disk I/O from userspace. 

\subsubsection{Create}
%\begin{figure}
%    \centering
%    \input{figures/evaluation/create}
%    \caption{Create Performance}
%    \label{fig:create}
%\end{figure}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
        & 1 Thread & 32 Threads \\ \hline
        \system{} & 1126 & 1072 \\ \hline
        C-Kernel & 933 & 881 \\ \hline
        FUSE & 24 & 24 \\ \hline
    \end{tabular}
    \caption{Create Microbenchmark Performance (Ops/sec)}
    \label{tab:create}
\end{table}

Performance for the file creation microbenchmark on an SSD is shown in \autoref{tab:create} for both single threaded and 32-threaded creates. In these benchmarks, \system{} shows competitive performance to the C version in the kernel and much better performance than the FUSE version. File creation involves many small writes (and so syncs in the log), so the FUSE performance is heavily impacted by slow syncs. FUSE shows less slowdown for creates than it does for writes. This occurs because the create microbenchmarks spend a smaller percentage of the time executing slow disk operations.

%Like \cite{tofuse}, we see very large performance degradation for creates. Many requests are generated, meaning many kernel crossing for the FUSE version, and neither batching nor caching are applicable. 

%Our evaluation shows even more performance degradation due to slow disk accesses. The overhead due to userspace disk I/O is particularly large for small writes since the \texttt{O\_DIRECT} file must be written to in block size chunks. File creation involves many small disk I/O for inode allocation, block allocation, parent directory modification, and file data writing, so the file creation benchmarks are particularly affected by this overhead.

\subsubsection{Delete}

% Deletes aren't included because the benchmark goes so quickly, it's difficult to trust the numbers at all.

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
        & 1 Thread & 32 Threads \\ \hline
        \system{} & 7499 & 7502 \\ \hline
        C-Kernel & 7500 & 8253 \\ \hline
        FUSE & 118 & 116 \\ \hline
    \end{tabular}
    \caption{Delete Microbenchmark Performance (Ops/sec)}
    \label{tab:delete}
\end{table}

Performance results for the file deletion microbenchmark on an SSD are shown in \autoref{tab:delete} for both single-threaded and 32-threaded benchmarks. These results show similar trends as the file creation microbenchmarks because both are metadata heavy benchmarks so generate many small writes.


\subsection{Macrobenchmarks}

\subsubsection{Varmail}
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
        & Varmail (ops/s) & Fileserver (ops/s) & Untar (s) \\ \hline
        \system{} & 320 & 3860 & 19.8 \\ \hline
        C-Kernel & 303 & 2947 & 31.6 \\ \hline
        FUSE & 24 & 7 & 3404.9 \\ \hline
        Ext4 & 785 & 5172 & 6.2 \\ \hline
    \end{tabular}
    \caption{Macrobenchmark Performance}
    \label{tab:macro}
\end{table}

%\begin{figure}
%    \centering
%    \input{figures/evaluation/varmail}
%    \caption{Varmail Macrobenchmark Performance}
%    \label{fig:varmail}
%\end{figure}

Performance results for the varmail macrobenchmark on an SSD are shown in \autoref{tab:macro}. The file system implemented using \system{} and the C version in the kernel have very similar performance while the FUSE version shows much worse performance. Since this is a metadata-heavy macrobenchmark, the xv6 file system results are similar to the metadata-heavy microbenchmarks (file creation and deletion). The FUSE version performs comparatively better on the varmal benchmark than it does on the other benchmarks because varmail executes fsyncs on files. While fsyncs are slower for the FUSE version than they are for the other two xv6 file systems, the slowdown is not as large when whole files are being synced instead of individual blocks. On all three versions of the xv6 file system, the fsyncs take up the majority of the runtime, so the performance properties of the fsyncs are reflected in the overall performance numbers. For this benchmark, ext4 performs about 2.5x faster than either of the in-kernel xv6 implementations.

\subsubsection{Fileserver}

%\begin{table}[]
%    \centering
%    \begin{tabular}{|c|c|}
%    \hline
%        \system{} & 3860 \\ \hline
%        C-Kernel & 2947 \\ \hline
%        FUSE & 7 \\ \hline
%        Ext4 & 5172 \\ \hline
%    \end{tabular}
%    \caption{Fileserver Macrobenchmark Performance (Ops/sec)}
%    \label{tab:fileserver}
%\end{table}

%\begin{figure}
%    \centering
%    \input{figures/evaluation/webserver}
%    \caption{Webserver Macrobenchmark Performance}
%    \label{fig:webserver}
%\end{figure}

Performance results for the fileserver benchmark on the SSD are shown in \autoref{tab:macro}. This benchmark involves many reads, writes, and file creates and deletes. Like the other benchmarks, these results show that the file system implemented using \system{} and the version using the VFS layer in the kernel have very similar performance, and both outperform the FUSE version. This benchmark is particularly affected by the FUSE slowdowns because it involves many writes and creates, both of which introduce significant overhead. Ext4 only performs only 33\% better than the xv6 file system written using \system{}. At that point, ext4 appears to be bounded by the throughput of the SSD.

\subsubsection{Untar Linux}

%\begin{table}[]
%    \centering
%    \begin{tabular}{|c|c|}
%    \hline
%        \system{} & 19.8 \\ \hline
%        C-Kernel & 31.6 \\ \hline
%        FUSE & 3404.9 \\ \hline
%        Ext4 & 6.2 \\ \hline
%    \end{tabular}
%    \caption{Untar Linux Macrobenchmark Performance (sec)}
%    \label{tab:untar}
%\end{table}

This benchmark (shown in \autoref{tab:macro}) untars the Linux kernel onto the relevant file system, generating many file creations and writes across many directories. Unlike the other benchmarks, this measures total execution time instead of operations per second, so lower is better. This benchmark shows somewhat more performance difference between the \system{} file system and the VFS file system. This is likely caused by the same difference seen in the write microbenchmarks: \system{} is able to batch sequential writes while the VFS implementation of xv6 is not.

%Like the other benchmarks, the file system version implemented using \system{} and the version implemented in C against the VFS layer have relatively similar performance, and the FUSE file system performs much worse. For this benchmark, ext4 executes the benchmark roughly 3x faster than the xv6 file system written using \system{}.

\subsection{Future Evaluation} \label{subsec:real-world}
As future work, we will demonstrate development velocity by implementing and evaluating real-world file systems using \system{}. The simplicity of the xv6 file system was ideal for the proof-of-concept work, but a more full-featured file system will better demonstrate the velocity, generality, and low performance impact of \system{}. We plan to focus on a research file system that shows promise for practical use, both proving that \system{} can support a more complicated file system and providing a high-performance implementation of a file system that has demand in the community.


%A practical extensibility framework for file systems must be able to support a wide variety of potential file system behavior. While we know that \system{} doesn't enable the level of fine-grained flexibility available using VFS, we still need to ensure that it provides sufficient functionality for many real-world file systems. Currently, we've only used the framework to implement the file system from xv6, a very simple file system. This simplicity was ideal for a proof-of-concept work, but doesn't show the generality of functionality that \system{} enables or evaluate the performance overhead \system{} may have for performance-critical file systems.

%In future work on this project, we will implement real-world file systems to demonstrate the flexibility enabled by \system{}. Given the breadth of file systems written using the FUSE API, we expect that \system{} will be able to support many different file systems. We plan to focus on a research file system that shows promise for practical use, both proving that \system{} can support a more complicated file system and providing a high-performance implementation of a file system that has demand in the community.

==> figures/design_fig.tex <==
\begin{tikzpicture} [node distance=1cm]
  \node (vfs) [kernel] {VFS};
  \node (fops) [framework, below of=vfs] {\system{}FS};
  \node (fs) [fs, below of=fops, yshift=-0.5cm] {File System};
  \node (kops) [framework, below of=fs, yshift=-0.5cm] {\system{}KS};
  \node (kern) [kernel, below of=kops] {Kernel Services};
  \draw [arrow] (vfs.220) -- (fops.140);
  \draw [arrow] (fops.40) -- (vfs.320);
  \draw [arrow] (fops.220) -- (fs.125);
  \draw [arrow] (fs.55) -- node[anchor=west] { \ding{\numexpr172\relax} File Operations API} (fops.320);
  \draw [arrow] (fs.235) -- (kops.140);
  \draw [arrow] (kops.40) -- node[anchor=west] { \ding{\numexpr173\relax} Kernel Services API} (fs.305);
  \draw [arrow] (kops.220) -- (kern.140);
  \draw [arrow] (kern.40) -- (kops.320);
\end{tikzpicture}

==> figures/user_design_fig.tex <==
\begin{tikzpicture} [node distance=1cm]
  \node (vfs) [kernel] {Posix};
  \node (fops) [framework, below of=vfs] {\system{}FS-User};
  \node (fs) [fs, below of=fops, yshift=-0.5cm] {File System};
  \node (kops) [framework, below of=fs, yshift=-0.5cm] {\system{}KS-User};
  \node (kern) [kernel, below of=kops] {clib};
  \draw [arrow] (vfs.220) -- (fops.140);
  \draw [arrow] (fops.40) -- (vfs.320);
  \draw [arrow] (fops.220) -- (fs.125);
  \draw [arrow] (fs.55) --  (fops.320);
  \draw [arrow] (fs.235) -- (kops.140);
  \draw [arrow] (kops.40) --  (fs.305);
  \draw [arrow] (kops.220) -- (kern.140);
  \draw [arrow] (kern.40) -- (kops.320);
\end{tikzpicture}

==> future.tex <==
\section{Future Work}
While we've made significant progress on developing a practical extensibility framework for Linux kernel file systems, there are still more features we plan to add. Our future work on this project will implement features to support the development process and real-world file systems using our framework, along with updating to recently released technology.

\subsection{Efficient Composition}
Efficient composition of file systems, where one file system is implemented as a layer on top of a lower file system, can also contribute to high development velocity. The ability to modify the behavior of a file system without rewriting the underlying file system can enable faster iteration, modular development, and more code reuse. Composable, or stackable, file systems can be implemented today using the VFS layer, but at significant performance cost. For the upper file system to make requests to the lower file system, it must pass through the entire VFS layer, adding significant overhead.

Our framework has the potential to enable efficient composition of file systems by providing explicit support for composable file systems. By providing an interface specifically for layered file systems and handling the modifications entirely within the framework, our framework could provide efficient, flexible support for composing file systems. In future work, we will design and implement this feature.

\subsection{Debugging API}
File systems, or any large piece of kernel code, is difficult to write correctly. Due to the potentially high impact of bugs in the operating system, kernel file systems must be thoroughly tested. Past works~\cite{crashmonkey,hydra} have proposed frameworks to support debugging kernel file systems. Our framework could implement the behavior described by those, or similar, systems, providing additional debugging support to file systems implemented using our framework.

%\subsection{Real-World File Systems}
%A practical extensibility framework for file systems must be able to support a wide variety of potential file system behavior. While we know that our framework doesn't enable the level of fine-grained flexibility available using VFS, we still need to ensure that the framework provides sufficient functionality for many real-world file systems. Currently, we've only used the framework to implement the file system from xv6, a very simple file system. This simplicity was ideal for a proof-of-concept work, but doesn't show the breadth of functionality that our framework enables.

%In future work on this project, we will implement a real-world file system to demonstrate the flexibility enabled by our framework. Given the breadth of file systems written using the FUSE API, it's expected that our framework will be able to support many different file systems. We plan to focus on a research file system that shows promise for practical use, both proving that our framework can support a more complicated file system and providing a high-performance implementation of a file system that has demand in the community.

%\subsection{Linux \texttt{io\_uring}}
%Recent versions of the Linux kernel have included a new abstraction for performing asynchronous I/O from userspace called \texttt{io\_uring}. This interface can be used to increase performance of userspace I/O since the user won't have to block on operations that don't need to be completed synchronously. Using this interface for the I/O accesses from the FUSE version of the xv6 file system in the evaluation could result in better performance numbers, potentially decreasing the overhead seen by using FUSE. More interestingly, our framework could hook into the file I/O part of \texttt{io\_uring} along with the VFS layer, allowing users to entirely bypass the VFS layer. We can't currently use \texttt{io\_uring} because our framework is built in Linux kernel version 4.15 and \texttt{io\_uring} wasn't introduced until kernel version 5.1. Updating to the new kernel version and incorporating \texttt{io\_uring} will be part of future work.


==> goals.tex <==


%\section{Goals}
%\todo{Give the goals their own section? They're in the background right now}

==> intro_old.tex <==
\section{Introduction}
High development velocity has become a widespread talisman for cloud software development~\cite{fbrelease}.
Many popular cloud systems roll out new software releases on a weekly or even daily basis, to give users faster access
to new features, to gain insight into priorities for further development, and to reduce integration costs.
While this design pattern may seem inappropriate for mission critical software, cloud vendors
have shown it is practical to use short release cycles for many high reliability services, including 
databases~\cite{spanner} and network stacks~\cite{andromeda,snap,catapult}.

Rapid release cycles have largely skipped the operating system kernel development community, however.  Linux
is the most widely used server operating system for the cloud, but new versions drop only every few months, 
with major changes limited to once every few years. Of course, Linux is open source, and so anyone is free to iterate
more rapidly, at the cost of the later pain of reintegration with the mainline development tree.

The Linux community has adopted several approaches to improving feature velocity, none entirely successful.
One approach is to try to future-proof the kernel by adding features before they are needed.  We can see that
in action with the popular Docker container manager~\cite{docker}. 
Docker leverages several recently-added Linux kernel features, but in the process exposed a number of potentially
critical flaws in those kernel services that could compromise the security of the entire operating system.  
Alternately, we can move kernel services to user level, such as with the FUSE file system abstraction~\cite{fuse} 
and Open vSwitch~\cite{openvswitch}.
However, these can impose a prohibitively high performance penalty~\cite{tofuse,ceph}, necessitating a kernel caching layer~\cite{extfuse} that poses its own set of tradeoffs.
Certain Linux kernel interfaces can be rapidly reconfigured with eBPF~\cite{ovs-ebpf} scripts, but only for small 
linear snippets of code.  
The widespread belief that in the future, all high performance operations must ``bypass the kernel''
is an illustration of how operating systems are losing the race~\cite{arrakis,ix,demikernel}.

Our goal is to enable high velocity development for high-performance, general-purpose operating system kernel 
extensions. Our trust model is that of a slightly harried kernel developer, rather than an untrusted application
developer. We want to provide a way for kernel developers
to add kernel features in a manner that isolates bugs to within the extension 
and also allows for dynamic replacement of that functionality
without the need to restart applications~\cite{barrelfish}.  To be as widely applicable as possible,
we focus on enabling rapid development of Linux kernel code, rather than to assume a new code base designed
for extensibility, such as Exokernels~\cite{exokernel}, Spin~\cite{spin}, or Barrelfish~\cite{barrelfish}.
To be concrete, we restrict ourselves, at first, to file system extensibility. We leave dynamic replacement of
file systems to future work.

%1) OS extensibility - the ability to easily and safely add features to an existing OS - is a long standing goal of OS design.  Although a large number of techniques have been proposed, no effective solution exists today for complex parts of performance-critical kernel functionality to be added in a safe manner.  
%As evidence, look at what happened with Docker - a clearly important piece of functionality that
%needed to be added quickly, but that also introduced a large number of critical bugs.  Or Snap, where a large OS dev effort to replace the TCP stack done entirely out of the kernel for velocity, even at the cost of compromising performance for a performance-critical service.

% Operating system extensibility - the ability to easily and safely add features to an existing operating system - is a long standing goal of operating system design. Although a large number of techniques have been proposed~\cite{sfi,lxfi,bpf,spin}, no effective solution exists today for complex parts of performance-critical kernel functionality to be added in a safe manner. For example, consider Docker. The kernel functionality it uses is clearly important and needed to be added quickly, but also also introduced a large number of critical bugs. Also, in Snap~\cite{snap} and Ceph~\cite{ceph}, significant development effort was done to replace the TCP stack and block storage layer, respectively, outside of the kernel for velocity, even at the cost of compromising performance.

% \todo{I'm not sure what to do with the Docker argument. As is, the argument you used in the intro outline talks about functionality integral to Docker's functioning, pieces of code that needed to be added so Docker could run and that were added specifically for Docker. I would think that would refer to cgroups and namespaces. I would believe that these have introduced critical bugs, but I'm not sure what to cite for that, and we didn't do the analysis on those. We analyzed three extensions that Docker uses, but weren't added specifically for Docker. Given that, the "clearly important" and "needed to be added quickly" arguments don't hold as much weight. I can either try to cite something for cgroups and namespaces, or we can shift the argument over to functionality used by Docker.}

%2) We argue that the reason is that there is no existing technology that provides all of the features for extensibility that we want:
%a) safety - define (carefully, since you aren't trying to sandbox extensions)
%b) performance - define, include tail performance (because that's part of the problem with GC)
%c) generality - define
%d) velocity - define
%e) works with existing OS'es - not greenfield

% \todo{I realize our discussion earlier today was slightly different from the goals mentioned here. The ability to debug code easily doesn't fit under any of the goals here, but it does seem important and worth discussing. It could go under velocity, but we decided that term is too broad and we should maybe have hot-swaps or something instead. Should we really have something like "testing/deployment features" to encompass the online/graceful reconfiguration and userspace debugging? I'm not sure what the elegant term for that would be. I'll make it two separate things for now, I guess}

% We argue that there is no existing technology that provides all of the features for extensibility that we would want: safety, performance, generality, graceful redeployment, easy debugging, and compatibility with existing operating systems. Safety - reducing bugs or their impact on the rest of the operating system - is necessary given the potentially catastrophic consequences of kernel bugs. Performance, including tail performance, must be high for performance critical use cases. Generality is needed to support the full range of possible extensions; the extensibility technology shouldn't overly limit the allowed behavior. Graceful redeployment provides the ability to redeploy extensions without disrupting other services, enabling fast release cycles that are needed for industry development. Debugging is both particularly difficult and particularly important for kernel code; extensions should be easy to debug. Compatibility with existing operating systems is necessary for the technology to be useful today, rather than after years of waiting for the new operating system to mature.

%3) Our approach is inspired by the availability of type-safe non-GC performant languages like Rust.  That addresses a,b,c.  But d+e are the hard part - how do we get this into a widely used existing OS like Linux, so that we don't have to wait another generation for a new OS to spring up built on better principles.  Here we can say Linux has spent a lot of effort on extensibililty - it isn't a foreign concept to Linux, but the options all have tradeoffs and we'd like a solution that could allow for new chunks of the OS to be injected safely without needing to reboot or run slowly.

Our approach is inspired by the recent availability of type-safe, non-garbage collected, performant languages like Rust. Writing kernel extensions in Rust eliminates a class of cross-module bugs that could compromise kernel security, without
the performance overhead of running at user-level or the restrictions on extension behavior imposed by eBPF. However, supporting compatibility with existing operating systems and features for high development velocity such as dynamic module replacement, debugging, and code reuse, is challenging. 
%However, supporting dynamic module replacement, debugging, and compatibility with existing systems is challenging. 

% It's important to integrate our approach with a widely-used existing operating system like Linux so it can be used in production systems today. The design of Linux focuses on extensibility, and past approaches~\cite{bpf,sfi,lxfi,fuse} have added enhanced this extensibility in various ways. However the existing options all have tradeoffs, either sacrificing safety, performance~\cite{fuse,sfi}, or generality~\cite{bpf}, and no approach provides graceful redeployment, either requiring shutdown of the relevant extension or a reboot of the machine, or built-in methods of debugging. We want to provide a solution that can allow new pieces of Linux to be injected into the operating system safely without needing to reboot the machine or run slowly.

%- How can we integrate this idea with an existing system, like Linux?
%- Linux focuses on extensibility, but the options have tradeoffs, either sacrificing safety, performance, or generality. 

%4) We've demonstrated by building a framework for injecting general-purpose file systems and file system extensions into Linux.  ...

%Extensibility has been a long-standing goal of operating systems research. This ability to modify the behavior of an operating system is critical to allowing the same codebase to be used in diverse environments. Linux has embraced this design principle, focusing on extensibility for both small pieces of code and whole modules. However, implementing extensions in Linux is still a slow and error-prone process~\cite{faults,snap}, discouraging developers from making full use of this feature. For an extensibility framework to support the needs of modern developers, it should provide several properties: high performance, high development velocity, and safety/resilience to bugs in the extensions, generality of allowed file systems, and usability.

%There have been a number of past approaches to supporting extensibility in Linux~\cite{bpf,lxfi,sfi}, but none of the existing approaches provide all of these features. The interfaces exposed by Linux provide very little safety, but techniques for ensuring safety come with either high performance or development overhead. Today, the majority of Linux extensions use no techniques for ensuring safety, leading to potentially dangerous behavior. For example, the file system used by Docker (Overlay Filesystem) has had a number of bugs that could result in kernel panics.

%We propose a framework that applies ideas from microkernel operating systems to extensions running in the Linux kernel. Our framework enforces modularity between the core kernel and the extensions by using an interface inspired by message-passing APIs. To enforce safety within the extensions, we rely on programming language techniques. Extensions must be written in a type-safe language without garbage collection, namely Rust, providing safety without performance overhead or performance unpredictability due to garbage collection. Our framework can provide features for fast development, such as live redeployment, allowing extensions to be updated without shutting down services relying on the extension.

For this work, we focus on high velocity kernel file systems.  We have built a framework, called Bento, for
injecting general-purpose file systems and file systems extensions, written in Rust, into Linux.
Surprisingly, Linux's existing pluggable file system interface, VFS, is poorly suited to our needs,
as it assumes shared data structures can pass freely across the extension interface, complicating compile-time
type checking. Instead, Bento interposes a thin layer for calls into the file system, and calls from the 
file system back into the kernel, providing safety, high performance, generality, and compatibility with Linux.
While our architecture is designed to be compatible with graceful online upgrades of running file systems along with support for other features for high development velocity, 
we leave that for future work.

% We've demonstrated this approach by building a framework for injecting general-purpose file systems and file systems extensions into Linux. \system{} enables running safe Rust file systems in the Linux kernel, providing safety, high performance, generality, and compatibility with Linux. We will implement graceful redeployment as we continue work on this project. The Linux kernel isn't designed for Rust's type-safety checks, so maintaining safety at the intersection of the kernel and file system, both for calls from the kernel to the file system and vice versa, is challenging. \system{} interposes a thin layer at both of these intersections, translating unsafe kernel interfaces into safe interfaces exposed to the file system.

%- the system enables running Rust file systems in the Linux kernel
%- Interfacing with Linux imposes a challenge for maintaining safety, both where the file system interacts with the VFS layer and where the file system interacts with kernel services, like the block storage layer.
%- Bento interposes a thin layer in both of these places, translating unsafe kernel interfaces into safe interfaces
%- At the VFS side, restrict memory sharing 
%- At the kernel services side, wrap kernel services in safe abstractions.

%In this project, we have implemented this proposal for file systems in Linux. We developed a shim layer in the kernel that executes between the file system and the surrounding layers of the kernel. The framework interposes between the VFS layer and the file systems, translating VFS calls to the interface exposed to file systems. We enforce an “ownership model” on this interface, allowing memory sharing as long as one side “owns” the memory while the other “borrows” the memory for a restricted time. Our framework additionally wraps kernel functionality needed by the file system, such as block I/O, in Rust wrappers, enabling the file system to use kernel functionality while being written primarily in the safe subset of Rust. We develop primitives to enable safety exposing this kernel functionality: opaque pointers to support exposing kernel data structures to the file system and memory wrappers to enable file system owned memory.

We have used \system{} to implement the xv6 file system to run in the Linux kernel. We have additionally implemented baseline versions, one written in C against the VFS layer and one (written in Rust) running in userspace using FUSE. We found that our framework has performance very similar to, and sometimes better than, the VFS C version while the FUSE version performed much worse than both.


In this paper, we make the following contributions:
\begin{itemize}
    \item We design and implement \system{}, a framework that enables high-velocity development of safe, performant file systems in Linux.
    \item We present techniques for allowing safe Rust code to run in the Linux kernel and access kernel functionality.
    \item We implement a file system using \system{} and evaluate its performance characteristics.
\end{itemize}


==> related_old.tex <==
\section{Related Work}

\subsection{FUSE}
FUSE (Filesystem in Userspace)~\cite{fuse} is a framework that enables implementing a file system to run in userspace. The FUSE framework consists of two pieces, a kernel driver that translates VFS calls to FUSE-internal requests that are sent to userspace and libFUSE, a userspace library that interfaces with the user file system. Like \system{}, FUSE targets safety and ease-of-development for Linux file systems. It’s able to provide these properties quite well by running code in userspace and providing a simplified interface. However, running the file system in userspace introduces extra kernel crossings, leading to up to 83\% overhead. This overhead is too severe for many applications, and production systems rarely employ FUSE. \system{} takes advantage of the interface work done in FUSE, using the FUSE low-level interface and a modified version of the FUSE kernel driver.

\subsection{eBPF}
The extended Berkeley Packet Filter (eBPF)~\cite{bpf} is another technique for safe extensibility in Linux. It allows users to insert limited pieces of code to run in the Linux kernel at a set of predefined locations with restricted permissions. As implied by the name, eBPF was originally aimed at network packet processing, but has since been expanded to support broader functionality. While the mainline eBPF code has no support for file systems, a project~\cite{extfuse} has enabled writing parts of a stackable file system using eBPF. Broadly, eBPF provides a high level of safety and good performance but can’t easily support the large modules with complex logic and data structures that \system{} targets. eBPF programs are limited in size and type of operations. While eBPF programs can be chained together with tail calls, maintaining state across the tail calls is complicated at best.

\subsection{Verification}
Over the last few years, several papers have been published on verified operating systems and file systems~\cite{hyperkernel,fscq,yggdrasil}. These projects use formal verification to ensure that an implementation of a system abides by some defined correctness properties. By enforcing proofs of correctness properties, this technique is able to eliminate many bugs without necessarily adding performance overhead. However, verified file systems are still difficult to design and implement, requiring specialized knowledge. Additionally, there are currently no practical mechanisms to verifying concurrent code.

\subsection{Software Fault Isolation}
Software fault isolation is a technique for limiting the impact of faults in a module and has seen several implementations~\cite{sfi,bgi}, including one for Linux modules~\cite{lxfi}. Using this technique, faults in a protected module are unable to impact the correctness of surrounding code. SFI can have significant performance overhead in many cases, ranging anywhere from 0$\times$ to 4$\times$ CPU overhead. This overhead manifests both while executing the isolated. module and while transitioning into and out of the module. Additionally, while SFI can address some of the safety concerns when developing Linux modules, it does not reduce the number of bugs in the module, only ensuring that bugs in the module will be isolated to the module.

\subsection{High-level Languages}
Other projects have also employed a high-level language with a strict type system to provide safety in the operating system. Like \system{}, the SPIN operating system~\cite{spin} provides safe extensibility by combining a safe, modular interface with modules implemented in a safe language, though SPIN designed the whole operating system around extensibility. \system{} applies these techniques and the associated benefits to Linux. Other operating systems projects, such as Singularity~\cite{singularity}, Biscuit~\cite{biscuit}, and Redox~\cite{redox}, explore writing the entire operating system in a high-level language. Additionally, we’re not the first group to integrate Rust code into the Linux kernel. Other projects have implemented device drivers in Rust~\cite{rust_devices,linux_module_rust}.


